InTAS -- The Ingolstadt Traffic Scenario for SUMO

Vehicular Ad Hoc Networks (VANETs) are expected to be the next big step towards safer road transport, supporting applications to exchange information between vehicles. To develop novel applications for this area a high number of tests, considering all traffic situations, are demanded. However, it is unfeasible to reproduce these tests in real life, by the fact that any failure on the applications would cause severe impacts on transport system safety and could risk human lives. Thus, this paper presents the concept, model, and validation for InTAS, a realistic traffic scenario for Ingolstadt. InTAS road topology accurately represents Ingolstadt real road map. Elements such as buildings, bus stops, and traffic lights were added to the map. Twenty traffic lights systems were simulated according to the real program deployed on the traffic lights. Traffic demand was modeled based on the activitygen method, considering demographic data and real-traffic information. The city public transport system was also simulated accordingly to bus time-tables and their routes. The simulation step was implemented considering the best value for device.rerouting.probability, which was defined by evaluating InTAS output and real traffic data. The scenario was validated by comparing real-traffic data from 24 measurement points with InTAS simulation results.

==> comments.tex <==

----------------------- REVIEW 1 ---------------------
SUBMISSION: 24
TITLE: InTAS - The Ingolstadt Traffic Scenario for SUMO
AUTHORS: Silas Lobo, Stefan Neumeier, Evelio Fernandez and Christian Facchi

----------- Overall evaluation -----------
SCORE: 3 (strong accept)
----- TEXT:
This paper is well organized and the scenario development is described in great detail so that it was easy to understand.

With the figures, a legend on the figure would be good and not just a description in the text. --- CLOSED



----------------------- REVIEW 2 ---------------------
SUBMISSION: 24
TITLE: InTAS - The Ingolstadt Traffic Scenario for SUMO
AUTHORS: Silas Lobo, Stefan Neumeier, Evelio Fernandez and Christian Facchi

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
This paper presents a realistic traffic scenario for Ingolstadt - covering the road network, traffic lights and traffic demand. The need for a new traffic scenario is well argued - especially with regard to the context of VANET research. The text is well structured and generally well written. Thank you for making this scenario publicly available!

Remarks:
- page 2
  - please use the sumo reference publication (https://elib.dlr.de/124092/) -- DONE

- page 5
  - Was there a particular reason, why you chose not to correct the errors in OpenStreetMap - since it is an "open source project working on the wiki style process"? -- TODO
 
- page 11
  - Did you use public transport data in the GTFS format?
  -- IGNORED

- page 13
  - "This attitude happens" - "This setting becomes effective ..." -- DONE

- page 18
  - "Additionally, a QQPlot test was implemented" -- DONE
  - "The authors would also like to thank ..." -- DONE



----------------------- REVIEW 3 ---------------------
SUBMISSION: 24
TITLE: InTAS - The Ingolstadt Traffic Scenario for SUMO
AUTHORS: Silas Lobo, Stefan Neumeier, Evelio Fernandez and Christian Facchi

----------- Overall evaluation -----------
SCORE: 3 (strong accept)
----- TEXT:
#Page 2:
- It's Vila Real not Vila Rica -- DONE
---------------

#Page 7:
- "Those 13 parking areas were tracked during an average usage at business days between Tuesday to Thursday, from September to December." -> Maybe you should specify which year. -- Checked

- You say that parking lot P1 was considered "always full", but in table 2 it doesn't look full (specially P1 Tiefgarage Theater Ost). Maybe you should change the sentence or correct the table. -- DONE
---------------

#Other:

- Figure 7 and Figure 9 need a legend, explaining the colors within the figure (i know that it is explained in the text, but it is always better to put it on the figure too). -- DONE


Overall, it's a good job and it would be great if you keep improving the scenario, as you mention.








----------------------IMPROVEMENTS FROM MY VIEW--------------------

01. Comment about the type of streets inserted for Car2X communication



Table~\ref{tab:publicparking} lists those parking areas and compares their total capacity with the average number implemented in InTAS.
The parking areas currently closed for construction work "P2" and P8" were considered to be always full, which partly reflects their usage before getting closed.


\begin{table}[tb]\small
\begin{center}
  \begin{tabular}{lcc}
   \hline
    Parking Area Name                   & Total Capacity    & Implemented Capacity \\
   \hline
    P1 Tiefgarage Theater West          & 398               &  345 \\ 
    P1 Tiefgarage Theater Ost           & 388               &  282 \\
    P2 Tiefgarage Schloß                & 448               &  448 \\
    P3 Tiefgarage Münster               & 207               &  151\\
    P4 Tiefgarage Reduit Tilly          & 281               &  130 \\
    P5 Parkplatz Hallenbad              & 612               &  507 \\
    P6 Parkplatz Festplatz              & 1,287             &  723 \\
    P7 Parkplatz Südl. Ringstraße       & 244               &  178 \\
    P8 Parkhaus Hauptbahnhof West       & 811               &  811 \\
    P9 Parkhaus Hauptbahnhof Ost        & 185               &  184 \\
    P10 Parkhaus Nordbahnhof            & 232               &  166 \\
    P11 Congressgarage                  & 375               &  222 \\
    P12 Tiefgarage Zeughaus             & 100               &  100 \\
   \hline
  \end{tabular}
\end{center}
\normalsize
\caption{Comparison of real capacity parking areas with used in InTAS~\cite{parkingareas} 
  \label{tab:publicparking}}
\end{table}
